Sketch and Project: Randomized Iterative Methods for Linear Systems and Inverting Matrices

Probabilistic ideas and tools have recently begun to permeate into several fields where they had traditionally not played a major role, including fields such as numerical linear algebra and optimization. One of the key ways in which these ideas influence these fields is via the development and analysis of randomized algorithms for solving standard and new problems of these fields. Such methods are typically easier to analyze, and often lead to faster and/or more scalable and versatile methods in practice. This thesis explores the design and analysis of new randomized iterative methods for solving linear systems and inverting matrices. The methods are based on a novel sketch-and-project framework. By sketching we mean, to start with a difficult problem and then randomly generate a simple problem that contains all the solutions of the original problem. After sketching the problem, we calculate the next iterate by projecting our current iterate onto the solution space of the sketched problem.

==> Frontmatter/abv.tex <==
\singlespacing
\addcontentsline{toc}{chapter}{List of Abbreviations}% Adds the title "List of Abbreviations"
\chapter*{List of Abbreviations \markboth{List of Abbrevations}{}}
% to get "List of Abbrevations" into the header 
\small
\begin{tabular}{ll}
	ASAP & As soon as possible \\
	RDY & Ready\\
\end{tabular}\\ [6pt]
\clearpage

==> Frontmatter/publications.tex <==
\singlespacing
\addcontentsline{toc}{chapter}{Author's Publications}
\chapter*{Author's Publications  \markboth{Author's Publications}{}}
\vspace{.3in}
\begin{spacing}{1.6}
\noindent
\small
 % University of Edinburgh mandatory declaration
During the course of the PhD program the candidate has co-authored six papers~\cite{Gower2012Sparsity,Gower2013,Gower2014c,Gower2015,Gower2015c,Gower2016}, all of which he was the first author and main contributor. This thesis is based on three of these papers, with a one-to-one correspondence between a chapter and a paper according to the following table.
\begin{center}
\begin{tabular}{|c||ccc|} \hline
Chapter & \ref{ch:linear_systems} & \ref{ch:SDA} & \ref{ch:inverse} \\ \hline
Paper & \cite{Gower2015} & \cite{Gower2015c} & \cite{Gower2016} \\ \hline
\end{tabular}
\end{center}


\vspace{1.75in}
\noindent
Robert Mansel Gower\\ % author's name
29th of February 2016 % date of submission
\end{spacing}
\clearpage

